Combining Representation Learning with Logic for Language Processing

The current state-of-the-art in many natural language processing and automated knowledge base completion tasks is held by representation learning methods which learn distributed vector representations of symbols via gradient-based optimization. They require little or no hand-crafted features, thus avoiding the need for most preprocessing steps and task-specific assumptions. However, in many cases representation learning requires a large amount of annotated training data to generalize well to unseen data. Such labeled training data is provided by human annotators who often use formal logic as the language for specifying annotations. This thesis investigates different combinations of representation learning methods with logic for reducing the need for annotated training data, and for improving generalization.

==> 3_legacy.tex <==
\comment{
\subsubsection{Full-rank Logic}
\todoc{shorten!}
\todoc{we need a precise definition what we mean by the term low-rank logic}

\rockt{move grefenstette isomorphism to related work and directly start with full-rank vector embeddings of relations}
\newcite{grefenstette2013towards} showed that first-order logic is isomorphic to a tensor calculus where logical statements evaluating to $\lTrue$ or $\lFalse$ are mapped to $[\lTrue] := \tTrue^T$  and $[\lFalse] := \tFalse^T$ respectively.
Let $|\mathcal{D}|$ be the size of the domain of entities, then every entity can be encoded by a $|\mathcal{D}|$-dimensional one-hot vector and every unary relation by a $|\mathcal{D}| \times 2$ matrix whose $i$th column is a truth vector encoding whether the $i$th entity in the domain belongs to that relation or not. 
Using this representation, $n$-ary boolean operators can be represented as mode-$(n+1)$ tensors.

Note that this isomorphism also holds if we represent each entity-pair $(e_i,e_j) \in \mathcal{P}$ as $|\mathcal{P}|$-dimensional vector and binary relations as $|\mathcal{P}| \times 2$ matrices. 
Furthermore, we can also represent $\lTrue$ and $\lFalse$ as $1$ and $0$, entity-pairs and relations as $|\mathcal{P}|$-dimensional one-hot and binary vectors respectively and use logical operators that operate one $1$ and $0$.
Hence, we can think of a trivial factorization of our $\mathcal{P} \times \mathcal{R}$ data matrix $\mathbf{T}$ as $\mathbf{T} = \mathit{I}\mathbf{R}$ where $\mathit{I}$ is the $\mathcal{P} \times \mathcal{P}$ identity matrix of one-hot entity-pair vectors and $\mathbf{R}$ in general is a \emph{full-rank} $\mathcal{P} \times \mathcal{R}$ matrix of relation vectors that memorize for which entity-pairs the relation holds. 
We call logic that operates on such representations of entity-pairs and relations \emph{full-rank logic}. 
Given a set of consistent first-order formulae, one can imagine how to change the entries in the relation vectors to fulfill these formulae.
}



%Consider a set of training data $\set{T} = \{(r_s(e_i,e_j), y_{sij})\}$ where $r_s(e_i,e_j)$ is a ground fact and $y_{sij}$ the corresponding ground truth, \ie{}, $1$ for known facts and $0$ for sampled unknown facts.
%\begin{equation}
%  \label{eq:9}
%  \loss{} = \sum_{r_s(e_i,e_j), y_{sij}\ \in\ \set{T}} - y\log(\ldiff{r_s(e_i,e_j)}) - (1-y)\log(1-\ldiff{r_s(e_i,e_j)}
%\end{equation}



% Given the notation presented above, matrix factorization can now be seen as a learning task in which low-dimensional embeddings are estimated for all constant pairs in $\mathcal{P}$ and predicates (relations) in $\mathcal{R}$, given a collection of ground atoms (facts) as supervision.
% We represent constant-pairs as rows and predicates as columns of a $|\mathcal{P}|\times|\mathcal{R}|$ binary matrix, and each atom in the training data represents an observed cell in this matrix.
% As introduced in \citet{riedel2013relation}, we seek to find a low-rank factorization into a $|\mathcal{P}| \times k$ matrix of embeddings of constant-pairs and a $k \times |\mathcal{R}|$ matrix of predicate embeddings such that they approximate the observed matrix.
% %\seb{This is somewhat sloppy, it's the natural parameters that are factorized. Can this sentence be removed? }
% %their dot-product (possible after application of the sigmoid function) accurately  %(Figure~\ref{fig:mf}).

% More precisely, let $\emb{(\cdot)}$ denote the mapping from constant-pairs and predicates to their corresponding embedding. That is, $\emb{r_m}$ is the embedding for predicate $r_m$, and $\emb{(e_i,e_j)}$ is the embedding for the pair of constants $(e_i,e_j)$. Let $\mathbf{w}$ be a possible world (\ie{} a set of ground atoms), and $\mathbf{V}$ be the set of all entity-pair and relation embeddings. Further, let $\pi_m^{e_i,e_j}=\sigma(\emb{r_m} \cdot \emb{e_i,e_j})$ where $\sigma$ is the sigmoid function and $\emb{r_m} \cdot \emb{(e_i,e_j)}$ denotes the vector dot-product between the embeddings of relation $r_m$ and entity-pair $(e_i,e_j)$. We define the conditional probability of a possible world $\mathbf{w}$ given embeddings $\mathbf{V}$ as 
% %$
% %{\small
% \begin{align*}
% p(\mathbf{w}|\mathbf{V}) &= \prod_{r_m(e_i,e_j) \in w} \pi_m^{e_i,e_j}\prod_{r_m(e_i,e_j) \notin w}\left(1-\pi_m^{e_i,e_j}\right).
% \end{align*}
% %}
% %$ 
% %where . 
% %From here on we will omit the $\mathbf{V}$ subscript for the $[\:]$ operator, and will later show how $[\:]$ can be extended to more complex formulae. 
% The embeddings can be estimated by maximizing the likelihood of a set of observed ground atoms  with $\ell_2$ regularization~\citep{collins2001generalization}, optimized using stochastic gradient descent.
% In summary, with atomic formulae (\ie{} factual knowledge) we learn entity-pair and relation embeddings that reconstruct known facts and are able to generalize to unknown facts. %\seb{we never mention how/why they generalize} 



%Thus, $[r_m(e_i,e_j)]$ has probability $1.0$ if the dot product between the two embeddings approaches infinity.
%
% This setting 
% corresponds to recent
% work in link prediction and relation extraction  
% recent work 
%
% For each observed pair of entities $p$ being in relation $R$, we introduce a factual constraint with 
% \[\denote{\mathcal{F}_{(p,R)}} \defeq \emb{R(p)} = \top.\]
% % and define the objective in \autoref{obj} over the sum of such factual constraints.
% Let
% \begin{align*}
%   %\mathcal{F} &:= r_m(e_i,e_j)\\
%   \eta_{\lForm,\gamma} &:=
%   \begin{cases}
%     -[\lForm]^{-1} &\text{if } \gamma = [\text{true}]\\
%     (1 - [\lForm])^{-1} &\text{if } \gamma = [\text{false}] 
%   \end{cases}
% \end{align*} 
% and note that
% \begin{align*}
%   \frac{\partial [\mathcal{F}]}{\partial \emb{e_i,e_j}} &= \frac{\partial \sigma(\emb{r_m} \lcdot \emb{e_i,e_j})}{\partial \emb{e_i,e_j}}\\
%   &= [\mathcal{F}]\left(1-[\mathcal{F}]\right)\emb{r_m}\\
%   \frac{\partial [\mathcal{F}]}{\partial \emb{r_m}} &= [\mathcal{F}]\left(1-[\mathcal{F}]\right)\emb{e_i,e_j}.
% \end{align*}
% Then the gradients with respect to entity-pair
% embedding $\denote{(e_i,e_j)}$ and relation embedding $\denote{r_m}$ are 
% \begin{align*}
%   \frac{\partial \mathcal{L}([\lForm],\gamma)}{\partial \emb{e_i,e_j}} &= \eta_{\lForm,\gamma}\frac{\partial [\mathcal{F}]}{\partial \emb{e_i,e_j}}\\
%   &= \eta_{\lForm,\gamma}[\mathcal{F}](1-[\mathcal{F}])\emb{r_m}\\ %&= ([r(e)] - 1) [r]\\ 
%   &=
%   \begin{cases}
%     -(1 - [\mathcal{F}]) \emb{r_m} &\text{if } \gamma = [\text{true}]\\
%     [\mathcal{F}]\emb{r_m} &\text{if } \gamma = [\text{false}]\\
%   \end{cases}\\
%   \frac{\partial \mathcal{L}([\lForm],\gamma)}{\partial \emb{r_m}} &= \eta_{\lForm,\gamma}\frac{\partial [\mathcal{F}]}{\partial \emb{r_m}}.
% \end{align*}

%From a collaborative filtering point-of-view these embeddings capture various correlations between the relation and the entity-pairs, \ie{}, entity-pairs similar according to their embeddings tend to be in similar relations and similar relations tend to hold for similar entity-pairs.
%The factorization model is quite attractive for relation extraction as it is not only able to accurately represent a variety of dependencies between the textual patterns and KB relations, but at the same time models dependencies between the patterns themselves, thus utilizing unlabeled data.

%One problem with the objective above is that it assumes positive as well as negative training facts. 
%In practice negative facts are often not present and one has to resort to sampling unobserved facts as negative facts.
%As alternative to the proposed objective  one could use a ranking objective which favors embeddings that lead to observed facts getting a higher predicted score than unobserved ones \citep{rendle09bpr}; \citep{riedel2013relation}.
%\rockt{..however, this would make our life hard regarding low-rank logic}




%\subsection{Low-Rank Logic Embeddings}
%\label{sec:bg:logicmf}
%
%Matrix factorization models are capable of learning complex dependencies between relations, however they rely on observed facts as training signal.
%For many relations in practice, however, the available distant labels may be insufficient to learn such dependencies due to the lack of quality alignments.
%In this paper we investigate whether the factorization can be learned when such dependencies are directly specified as first-order logic formulae. % encoding auxiliary background information.
%%In this section, we explore some of the dependencies that can be captured by the factorization models.
%%In other words, we are concerned with \emph{low-rank logic embeddings}, \ie{}, the $k$-dimensional dense vector representations of constants and predicates, where $k$ is much smaller than the number of constants or predicates, that represent first-order logical dependencies.
%In other words, we seek to learn \emph{low-rank logic embeddings} of predicates and constants, \ie{}, embeddings that lead to predictions which are consistent with provided first-order logical dependencies (see Figure~\ref{fig:mf}).
%More formally, given a partially observed binary matrix of ground facts and a set of logic formulae, low-rank logic embeddings are $k$-dimensional dense vectors that, when used to complete the matrix, respect both the observed ground facts, and at the same time, satisfy provided first-order logic formulae.
%
%%Formally, given a partially observed binary matrix of ground facts and a set of logic formulae, low-rank logic embeddings are those whose completion of the matrix respects both the observed ground facts, and at the same time, satisfies the logic formulae.
%%We seek to find $k$-dimensional dense vectors for relations and entity-pairs that reconstructs known facts and generalize towards unobserved facts (like in matrix factorization), but also follows the given formulae.
%
%%In particular, we are interested in dependencies encoded in the relation embeddings that would generalize to unseen facts, as opposed to dependencies encoded as a combination of relation and entity-pair embeddings, which is akin to memorization and does not necessarily generalize.
%
%Now that we have defined low-rank logic embeddings, the main question left to address is how such embeddings can be estimated.
%%Given that the observed ground facts are quite sparse, it is not clear whether such complex relations can be captured by matrix factorization on distant supervision data alone, especially for relations for which very few or no observed textual mentions are observed.
%In the next section, we propose such approaches that can utilize auxiliary sources of logical knowledge as external supervision to inject logical dependencies from these sources directly into the embeddings.






\subsubsection{Symmetric Equivalence}
It is quite straightforward to see how the similarity of relation embeddings directly capture the strength of correlations between relations.
If the embeddings of two relations $r_A$ and $r_B$ are identical ($\emb{A}=\emb{B}$), then for any entity pair $(e_i,e_j)$ the predictions $r_A(e_i,e_j)$ will be same as $r_B(e_i,e_j)$, and capturing the equivalence $\forall X, r_A(X)=r_B(X)$. 
We can trivially also show that embeddings can encode $\forall X, r_A(X)=\sneg r_B(X)$ by setting $\emb{A}=-\emb{B}$.
%\sameer{verify!}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}[b]{0.3\textwidth}
    \begin{tikzpicture}
      \scale{0.5}{
        \node[anchor = east] at (0,1.25) {$x_2$};
        \node[anchor = north] at (1.25,0) {$x_1$};
        \coordtwo
        \path[vector, color=blue] (0.center) -- node[at end, anchor = west] {$\mathbf{v}_\text{employeeAt}$} (2.2,3);
        \path[vector, color=red] (0.center) -- node[at end, anchor = west] {$\mathbf{v}_\text{profAt}$} (1.4,1.3);
      }
    \end{tikzpicture}
    \caption{Relation Embeddings}
    \label{fig:asymmetric:rels}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\textwidth}
    \begin{tikzpicture}
      \scale{0.5}{
        \node[anchor = east] at (0,1.25) {$x_2$};
        \node[anchor = north] at (1.25,0) {$x_1$};
        \coordtwo
        \path[vector, color=blue] (0.center) -- node[at end, anchor = west] {$\mathbf{v}_\text{employeeAt}$} (2.2,3);
        \path[vector, color=red] (0.center) -- node[at end, anchor = north west] {$\mathbf{v}_\text{profAt}$} (1.4,1.3);
        \path[vector, color=black] (0.center) -- node[at end, anchor = north west] {$\mathbf{v}_\text{XY}$} (3.0,2.4);
      }
    \end{tikzpicture}
    \caption{profAt $\simpl$ employeeAt} 
    \label{fig:asymmetric:impl}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\textwidth}
    \begin{tikzpicture}
      \scale{0.5}{
        \node[anchor = east] at (0,1.25) {$x_2$};
        \node[anchor = north] at (1.25,0) {$x_1$};
        \coordtwo
        \path[vector, color=blue] (0.center) -- node[at end, anchor = west] {$\mathbf{v}_\text{employeeAt}$} (2.2,3);
        \path[vector, color=black] (0.center) -- node[at end, anchor = south] {$\mathbf{v}_\text{XY}$} (0.9,1.6);
        \path[vector, color=red] (0.center) -- node[at end, anchor = west] {$\mathbf{v}_\text{profAt}$} (1.4,1.3);
      }
    \end{tikzpicture}
    \caption{Converse not necessarily true}
    \label{fig:asymmetric:reverse}
  \end{subfigure}
  \caption{\small{\bf Asymmetric reasoning:} Here we show an example of how an asymmetric implication relation profAt(X,Y)$\simpl$employeeAt(X,Y) can be captured by the relation embeddings in (a). In (b), we see that an entity embedding that has a high score for profAt will also have a high score for employeeAt, but in (c) we see that an entity pair for which employeeAt holds does not necessarily imply profAt as well.}
  \label{fig:asymmetric}
\end{figure*}


\subsubsection{Asymmetric Reasoning}
A quite useful relation that we would like the model to capture is the asymmetric implication relation, $\forall X, r_A(X)\simpl r_B(X)$.
Such dependencies occur quite often in real-world relation extraction data, for example we expect profAt($X,Y$) to imply employeeAt($X,Y$), but not the other way round.
In Figure~\ref{fig:asymmetric} we show how relation embeddings itself are able to capture such dependencies, in a way that for any entity-pair embedding $(e_i,e_j)$, if $r_A(e_i,e_j)$ is true then $r_B(e_i,e_j)$ is also true (Figure~\ref{fig:asymmetric:impl}), but $r_B(e_i,e_j)$ may be true without necessarily implying $r_A(e_i,e)j)$  (Figure~\ref{fig:asymmetric:reverse}).
%Every $\mathbf{v}_{(X,Y)}$ that has a high score for profAt(X,Y) will also have a high score for employeeAt(X,Y) but not vice versa.
%\sameer{more details?}
%\rockt{can we back this up experimentally?}

\subsubsect{Conjunctive Dependencies}
To encode basic conjunctions between relations $\forall X, r_A(X)\sand r_B(X)=r_C(X)$, we can set $\emb{C}=\emb{A}+\emb{B}$, where $\emb{A}\neq\emb{B}$.
Then for an entity pair $(e_i,e_j)$ for which both $r_A(e_i,e_j)$ and $r_B(e_i,e_j)$ is true, it is clear that $\emb{e_i,e_j}$ has to lie \emph{between} $\emb{A}$ and $\emb{B}$, and thus $r_C(e_i,e_j)$ will be true as well.
Disjunctions can be similarly encoded by setting the magnitude of $\emb{e_i,e_j}$ to be really large, such that it gives a positive prediction for $r_C(e_i,e_j)$ if \emph{either} $r_A$ or $r_B$ holds.
\sameer{verify!}
}




% \paragraph{Transitive Reasoning}
% \begin{figure}[t!]
%   \centering
%   \begin{tikzpicture}[scale=0.6]
%     % Interesting cells
%     \fill[color=cyan!20] (1,3) rectangle (2,4);
%     \fill[color=cyan!20] (4,3) rectangle (5,4);
%     \fill[color=cyan!20] (0,2) rectangle (1,3);
%     \fill[color=cyan!20] (1,2) rectangle (2,3);
%     \fill[color=cyan!20] (0,0) rectangle (1,1);
%     \fill[color=blue!20] (4,0) rectangle (5,1);

%     \draw[thick] (0, 0) grid (5, 4);

%     % Traning Data
%     % Row 1
%     \node at (1.5, 3.5) {1};
%     \node at (2.5, 3.5) {1};
%     \node at (4.5, 3.5) {1};
%     % Row 2
%     \node at (0.5, 2.5) {1};
%     \node at (1.5, 2.5) {1};
%     % Row 3
%     \node at (1.5, 1.5) {1};
%     \node at (3.5, 1.5) {1};
%     % Row 4
%     \node at (0.5, 0.5) {1};
%     \node at (4.5, 0.5) {0.8};

%     \fill[orange!10] (6,0) rectangle (8,4);
%     \draw[thick, color = orange] (6, 0) grid (8, 4);

%     \fill[red!10] (0,-1) rectangle (5,-3);
%     \draw[thick, color = red] (0, -1) grid (5, -3);

%     % Embeddings of constants
%     \node[anchor = west, color = black] at (8, 3.5) {$\mathbf{v}_\text{(Petrie, UCL)}$};
%     \node[anchor = west, color = black] at (8, 2.5) {$\mathbf{v}_\text{(Ferguson, Harvard)}$};
%     \node[anchor = west, color = black] at (8, 1.5) {$\mathbf{v}_\text{(Andrew, Cambridge)}$};
%     \node[anchor = west, color = black] at (8, 0.5) {$\mathbf{v}_\text{(Trevelyan, Cambridge)}$};
%     % Embeddings of relations
%     \node[anchor = west, rotate = -30, yshift=-5pt] at (0.5, -3) {$\mathbf{v}_\text{X-is-historian-at-Y}$};
%     \node[anchor = west, rotate = -30, yshift=-5pt] at (1.5, -3) {$\mathbf{v}_\text{X-is-professor-at-Y}$};
%     \node[anchor = west, rotate = -30, yshift=-5pt] at (2.5, -3) {$\mathbf{v}_\text{X-musuem-at-Y}$};
%     \node[anchor = west, rotate = -30, yshift=-5pt] at (3.5, -3) {$\mathbf{v}_\text{X-teaches-history-at-Y}$};
%     \node[anchor = west, rotate = -30, yshift=-5pt] at (4.5, -3) {$\mathbf{v}_\text{employeeAt(X,Y)}$};

%     % Connections
%     % Petrie, UCL
%     \draw[ultra thick, color=cyan, opacity=0.7] (1.5,-1) -- (6,3.5);
%     \draw[ultra thick, color=cyan, opacity=0.7] (4.5,-1) -- (6,3.5);
%     % Ferguson, Harvard
%     \draw[ultra thick, color=cyan, opacity=0.7] (0.5,-1) -- (6,2.5);
%     \draw[ultra thick, color=cyan, opacity=0.7] (1.5,-1) -- (6,2.5);
%     % Trevelyan, Cambridge
%     \draw[ultra thick, color=cyan, opacity=0.7] (0.5,-1) -- (6,0.5);

%     \draw[ultra thick, dashed, color = cyan] (0, -3) rectangle (1,-1);
%     \draw[ultra thick, dashed, color = cyan] (1, -3) rectangle (2,-1);
%     \draw[ultra thick, color = cyan] (4, -3) rectangle (5,-1);
%     \draw[ultra thick, dashed, color = cyan] (6, 3) rectangle (8,4);
%     \draw[ultra thick, dashed, color = cyan] (6, 2) rectangle (8,3);
%     \draw[ultra thick, color = cyan] (6, 0) rectangle (8,1);

%   \end{tikzpicture}
%   \caption{Transitive reasoning \todoc{make sure this makes sense when printed black and white!} \todoc{this figure might be omitted}}
%   \label{fig:transitive}
% \end{figure}

\section{Injecting First-order Logic}

Matrix factorization is capable of learning complex dependencies between relations, but requires observed facts as training signal. However, often we either do not have this signal because the relations of interest do not have pre-existing facts, or this signal is noisy due to alignment errors or mismatches when linking knowledge base entities to mentions in text. %\seb{or there simply is no mention of related entities in text?} 

To overcome this problem we investigate the use of first-order logic background knowledge (\eg{} implications) to aid relation extraction. 
One option is to rely on a fully symbolic approach that exclusively uses first-order logic~\citep{bos2005recognising,baader2007completing,bos2008semantics}. 
In this case incorporating additional background knowledge is trivial. However, it is difficult to generalize and deal with noise and uncertainty in language when relying only on manual rules. 
%\rockt{and cannot take advantage of the huge amount of unstructured text (\ie{} patterns and correlations between them)}
In contrast, matrix factorization methods can overcome these shortcomings, but it is not clear how they can be combined with logic formulae.
%\rockt{can we say why?}

In this section, we propose to inject formulae into the embeddings of relations and entity-pairs, \ie{}, estimate the embeddings such that predictions based on them conform to given logic formulae (see Figure~\ref{fig:mf} for an overview). 
We refer to such embeddings as \emph{low-rank logic embeddings}. 
Akin to matrix factorization, inference of a fact at test time still amounts to an efficient dot product of the corresponding relation and entity-pair embeddings, and logical inference is not needed.
%In the following we assume background knowledge in form of a set of logical formulae (see Table \ref{tab:formulae} for examples).
We present two techniques for injecting logical background knowledge, \emph{pre-factorization inference} (\S\ref{sec:pre-inference}) and \emph{joint optimization} (\S\ref{sec:low-rank-logic}), and demonstrate in subsequent sections that they generalize better than direct logical inference, even if such inference is performed on the \emph{predictions} of the matrix factorization model.



\subsection{Joint Optimization}
\label{sec:low-rank-logic}

\subsubsection{Training Objective}
\label{sec:objective}

Here we first present a learning objective that unifies ground atoms (facts) and logical background knowledge by treating both as logic formulae (atomic or complex), and define a loss function over this general representation.
We then define the loss function for ground atoms and simple implications, along with a brief sketch of how the loss can be defined for arbitrarily complex logic formulae.


\comment{
In the following we first present a general learning objective
that encourages distributed representations to behave like one-hot
representations under constraints. \rockt{with constraints we mean low-rank constraint here!?} Then we show how this objective can be optimized for
facts and implications.
\rockt{we might want to talk about predicates instead of relations and pairs of constants instead of entity-pairs}
}

As introduced in \S\ref{sec:bg:logic}, let $\mathcal{R}$ be the set of all relations/predicates and $\mathcal{P}$ be the set of all entity-pairs/constants.
Furthermore, let $\mathfrak{F}$ be a training set of logic formulae $\mathcal{F}$, %\comment{ and their target truth values $\gamma \in \{[\text{true}],[\text{false}]\}$}
and $\mathcal{L}$ a loss function. 
The training objective (omitting $\ell_2$ regularization on $\emb{(\cdot)}$ for simplicity) is  
 %\vskip -4mm
%\small
\begin{equation}
  \label{eq:obj}
  \min_{\mathbf{V}}
  \sum_{\mathcal{F} \in \mathfrak{F}} \mathcal{L}(\dFormula{F})
\end{equation}
 % \vskip -1mm
%Equation~\ref{obj} is general in that different representations of formulae, embeddings of entity-pairs and relations, as well as different loss functions can be used. 
where $\mathbf{V}$ is the set of all relation and entity-pair embeddings, and $\dFormula{F}$ is the marginal probability $p(w|\mathbf{V})$ that the formula $\mathcal{F}$ is true under the model. In this paper we use the logistic loss: $\mathcal{L}(\dFormula{F}) :=  -\log(\dFormula{F})$. The objective thus prefers embeddings that assign formulae a high marginal probability. 

%Precisely, the objective maximizes the likelihood of formulae that evaluate to [true] (or one minus the likelihood for formulae evaluating to [false]). 

To optimize this function we need the marginal probabilities $[\mathcal{F}]$, and the gradients of the losses $\mathcal{L}(\dFormula{F})$ for every $\mathcal{F}\in\mathfrak{F}$ with respect to entity-pair and relation embeddings, \ie{}, 
$\partial\mathcal{L}([\mathcal{F}])/\partial\emb{r_m}$ and $\partial\mathcal{L}([\mathcal{F}])/\partial\emb{(e_i,e_j)}$. 
Below we discuss how these quantities can be computed or approximated for arbitrary first-order logic formulae, with details provided for ground atoms and implications. %these for two types of formulae, ground atoms and first-order formulae, in detail, and outline how to extend the computation to arbitrary logic formulae.  
% vectors close to truth.  
% where $\vec{y} \in \left\{ \top, \bot \right\}$ is the ground-truth for $\mathcal{F}$.



\subsubsection{Ground Atoms}
\label{sec:ground-atoms}
% \paragraph{Objective}
Due to the conditional independence of ground atoms in the distribution $p(\mathbf{w}|\mathbf{V})$, the marginal probability of a ground atom $\mathcal{F} = r_m(e_i,e_j)$ is 
$[\mathcal{F}] =\pi_m^{e_i,e_j}=\sigma(\emb{r_m} \cdot \emb{e_i,e_j})$. Hence when only ground atoms (or literals) are used, objective \eqref{eq:obj} reduces to the standard log-likelihood loss.  
%
% \begin{align*}
%   \frac{\partial [\mathcal{F}]}{\partial \emb{e_i,e_j}} &= \frac{\partial \sigma(\emb{r_m} \lcdot \emb{e_i,e_j})}{\partial \emb{e_i,e_j}}\\
%   &= [\mathcal{F}]\left(1-[\mathcal{F}]\right)\emb{r_m}\\
%   \frac{\partial [\mathcal{F}]}{\partial \emb{r_m}} &= [\mathcal{F}]\left(1-[\mathcal{F}]\right)\emb{e_i,e_j}.
% \end{align*}
The gradients of the loss for the entity-pair
embedding $\emb{(e_i,e_j)}$ and relation embedding $\emb{r_m}$ are 
%\vspace{-1em}
%{\small
%  \vskip -4mm
\begin{align}
  \partial [\lForm]/\partial \emb{(e_i,e_j)} &= [\mathcal{F}](1-[\mathcal{F}])\emb{r_m}\\ %&= ([r(e)] - 1) [r]\\ 
  \partial [\lForm]/\partial \emb{r_m} &= [\mathcal{F}](1-[\mathcal{F}])\emb{(e_i,e_j)}\\ %&= ([r(e)] - 1) [r]\\ 
%\end{align}
%  \vskip -5mm
%\begin{align}
  \partial \mathcal{L}([\lForm])/\partial \emb{(e_i,e_j)} &= -[\mathcal{F}]^{-1} \partial [\lForm]/\partial \emb{(e_i,e_j)}\\ %&= ([r(e)] - 1) [r]\\ 
%  &=
%  \begin{cases}
%    -(1 - [\mathcal{F}]) \emb{r_m} &\text{if } \gamma = [\text{true}]\\
%    [\mathcal{F}]\emb{r_m} &\text{if }\gamma = [\text{false}]\\
%  \end{cases}\nonumber\\
  \partial \mathcal{L}([\lForm])/\partial \emb{r_m} &= -[\mathcal{F}]^{-1} \partial [\lForm]/\partial \emb{r_m}. %&= ([r(e)] - 1) [r]\\ .
\end{align}
% \vskip -5mm
%}
% \begin{align*}
%   \frac{\partial \mathcal{L}([\lForm],\gamma)}{\partial \emb{e_i,e_j}} &= \eta_{\lForm,\gamma}\frac{\partial [\mathcal{F}]}{\partial \emb{e_i,e_j}}\\
%   &= \eta_{\lForm,\gamma}[\mathcal{F}](1-[\mathcal{F}])\emb{r_m}\\ %&= ([r(e)] - 1) [r]\\ 
%   &=
%   \begin{cases}
%     -(1 - [\mathcal{F}]) \emb{r_m} &\text{if } \gamma = [\text{true}]\\
%     [\mathcal{F}]\emb{r_m} &\text{if } \gamma = [\text{false}]\\
%   \end{cases}\\
%   \frac{\partial \mathcal{L}([\lForm],\gamma)}{\partial \emb{r_m}} &= \eta_{\lForm,\gamma}\frac{\partial [\mathcal{F}]}{\partial \emb{r_m}}.
% \end{align*}
%The knowledge base may contain ground atoms (\ie{} facts) of the form $\mathcal{F}=r_m(e_i,e_j)$ for an entity-pair $(e_i,e_j)$ and a relation $r_m$. These atoms correspond to observed cells in a matrix where rows represent entity-pairs and columns represent relations. Learning fixed-length distributed representations that recover these facts corresponds to matrix
%factorization for %link prediction or 
%relation extraction and knowledge base completion~\cite{riedel2013relation}, which is an instance of generalized principle component analysis \cite{collins2001generalization}. \rockt{is this right?}

%Given a sparsely populated training matrix of $|\mathcal{R}|$ relations and $|\mathcal{P}|$ entity-pairs we seek to find a low-rank factorization into a $|\mathcal{P}| \times k$ matrix of entity-pair embeddings and a $k \times |\mathcal{R}|$ matrix of relation embeddings (see Figure \ref{fig:mf}). 



\subsubsection{First-order Logic}
Crucially, and in contrast to the log-likelihood loss for matrix factorization, we can inject more expressive logic formulae than just ground atoms. 
We briefly outline how to recursively compute the probability of the formula $[\mathcal{F}]$ and the gradients of the loss $\mathcal{L}([\mathcal{F}])$ for any first-order formula $\mathcal{F}$. Again, note that the probabilities of ground atoms in our model are independent conditioned on embeddings. This means that for any two formulae $\mathcal{A}$ and $\mathcal{B}$, the marginal probability of $[\mathcal{A} \wedge \mathcal{B}]$ can be computed as $[\mathcal{A}][\mathcal{B}]$ (known as \emph{product t-norm}), provided both formula concern non-overlapping sets of ground atoms. 
%In other words: the $[\;]$ operator for conjunction can be implemented as a  \emph{product t-norm}. The product t-norm,
%Evaluating the conjunction of two atoms using the multiplication of their scores is also referred to as .
In combination with $[\neg \mathcal{A}] := 1 - [\mathcal{A}]$ and the $[\;]$ operator as defined for ground atoms earlier, we can compute the probability of \emph{any} propositional formula recursively, \eg{},
%\vskip -5mm
%{\small
\begin{align*}
%$
  [\mathcal{A} \vee \mathcal{B}] &= [\mathcal{A}] + [\mathcal{B}] - [\mathcal{A}][\mathcal{B}]\\
  [\mathcal{A} \Rightarrow \mathcal{B}] &= [\mathcal{A}]([\mathcal{B}] - 1) + 1\\
  [\mathcal{A} \wedge \neg \mathcal{B} \Rightarrow \mathcal{C}] &= ([\mathcal{A}](1-[\mathcal{B}]))([\mathcal{C}] - 1) + 1.
%$
\end{align*}
%\vskip -1mm
%}
% $
%   [\mathcal{A} \vee \mathcal{B}] = [\mathcal{A}] + [\mathcal{B}] - [\mathcal{A}][\mathcal{B}],
%   [\mathcal{A} \Rightarrow \mathcal{B}] = [\mathcal{A}]([\mathcal{B}] - 1) + 1, \text{and}
%   [\mathcal{A} \wedge \neg \mathcal{B} \Rightarrow \mathcal{C}] = ([\mathcal{A}](1-[\mathcal{B}]))([\mathcal{C}] - 1) + 1.
% $
\noindent
Note that for statements $[\mathcal{F}]\in\{0,1\}$, we directly recover logical semantics. % ($0\equiv[\text{false}]$ and $1\equiv[\text{true}]$).
%For $[\:]\in[0,1]$, we now have an approach to compute the uncertainty of any formulae based on the uncertainty of its constituents.
First-order formulae in finite domains can be embedded through explicit grounding. For universal quantification we can get $[\forall x,y: \mathcal{F}(x,y)]=[\bigwedge_{x,y}\mathcal{F}(x,y)]$. If we again assume non-overlapping ground atoms in each of the arguments of the conjunction, we can simplify this to $\prod_{x,y}[\mathcal{F}(x,y)]$. When arguments do overlap we can think of this simplification as an approximation.   
%, and further assume closed world for tractability.
%\seb{grounding is mentioned both here and in the implication part. Can this be made less redundant?}

Since $[\mathcal{F}(x,y)]$ is defined recursively, we can back-propagate the training signal through the structure of $[\mathcal{F}]$ to compute $\partial[\mathcal{F}(x,y)]/\partial\emb{r_m}$ and $\partial[\mathcal{F}(x,y)]/\partial\emb{e_i,e_j}$ for any nested formula. %, and $\frac{\partial\mathcal{L}([\mathcal{F}],\gamma)}{\partial[\mathcal{F}]}$.
%\seb{the back propagation part still feels a little disconnected, can we omit it?}

\comment{
For $\mathcal{A},\mathcal{B} \in \{\text{true},\text{false}\}$ this recovers the semantics of logic.
However, with this formalism we can also reason over uncertainty, \eg{}, atoms that are predicted.
In the following we will take advantage of the fact that product t-norm formulae are differentiable and can thus be used to obtain gradients for the relation and entity-pair embeddings involved in the formula.

\todoc{probabilistic interpretation: A and B are assumed to be independent, therefore A and B = A*B}

For example, consider we have the formula $\mathcal{F} := r_s(e_i,e_j) \simpl r_t(e_i,e_j)$ and predictions
$r_s(e_i,e_j)=0.8$ and $r_t(e_i,e_j)=0.3$ for the two atoms, then $[r_s(e_i,e_j) \Rightarrow r_t(e_i,e_j)] = [r_s(e_i,e_j)]\left([r_t(e_i,e_j)] - 1\right) + 1 = 0.44$.
\todoc{alternative: {\L}ukasiewicz t-norm, but non-differentiable, therefore needs subgradients}
\todoc{connection to Grefenstette's Tensor Algebra: if you allow for truth values $[p\;\;(1-p)]^T$ and only look at the first component of truth vectors then his tensor operators are isomorphic to the product t-norm}
}


\subsubsection{Implications}
\label{sec:first-order-formulae}
A particularly useful family of formulae for relation extraction are universally quantified first-order formula over a knowledge base such as $\mathcal{F}=\forall x,y: r_s(x,y) \lImp r_t(x,y)$. 
Assuming a finite domain, such a formula can be unrolled into a conjunction of propositional statements of the form
%\resizebox{\columnwidth}{!}{
$\lForm_{ij} = r_s(e_i,e_j) \lImp r_t(e_i,e_j)$, one for each entity-pair $(e_i,e_j)$ in the domain. 
Specifically, $[\mathcal{F}]=\prod_{(e_i,e_j)\in\mathcal{P}}[\mathcal{F}_{ij}]$, and therefore $\mathcal{L}([\lForm])=\sum_{(e_i,e_j)\in\mathcal{P}}\mathcal{L}([\lForm_{ij}])$. %[\bigwedge_{(e_i,e_j)\in\mathcal{P}}\mathcal{F}_{ij}]=
%\footnote{We omit $\neg\forall x: [\mathcal{F}]$ here as it is equivalent to $\exists x: [\sneg\mathcal{F}]$. Existential quantification is rarely useful in practice, but we can derive a gradient using the product t-norm as well.}
%\todoc{as common in KBs, we can replace this conjunction by fulfilling each term individually, hence...} 
The gradients are derived as:
{\small
 % \vskip -5mm
\begin{align}
  [\lForm_{ij}] &= [r_s(e_i,e_j)]\left([r_t(e_i,e_j)] - 1\right) + 1\\
  \frac{\partial \mathcal{L}([\lForm_{ij}])}{\partial \emb{r_s}} &= -[\mathcal{F}_{ij}]^{-1} \left([r_t(e_i,e_j)] - 1\right) \frac{\partial [r_s(e_i,e_j)]}{\partial \emb{r_s}}\nonumber\\
  \frac{\partial \mathcal{L}([\lForm_{ij}])}{\partial \emb{r_t}} &= -[\mathcal{F}_{ij}]^{-1} [r_s(e_i,e_j)] \frac{\partial [r_t(e_i,e_j)]}{\partial \emb{r_t}}\\
  \frac{\partial \mathcal{L}([\lForm_{ij}])}{\partial \emb{e_i,e_j}} &= -[\mathcal{F}_{ij}]^{-1} \left([r_t(e_i,e_j)] - 1\right) \frac{\partial [r_s(e_i,e_j)]}{\partial \emb{e_i,e_j}}\nonumber\\
  &\quad-[\mathcal{F}_{ij}]^{-1}[r_s(e_i,e_j)]\frac{\partial [r_t(e_i,e_j)]}{\partial \emb{e_i,e_j}}.
  %&\hspace{5.5em}
\end{align}
 % \vskip -2mm
}
\noindent
Following such a derivation, one can obtain gradients for other first-order logic formulae as well.

%We are also interested in implications of the form $\mathcal{F}=\forall x,y: r_s(x,y) \lImp \sneg r_t(x,y)$ in order to, for example, correct the errors caused by spurious correlations in the data.
%Much of the above derivation remains the same for gradient computation, we just need to use the alternate definition of $[\mathcal{F}_{ij}]$ computed from the product t-norm. \sameer{remove this para?}

\comment{
\rockt{double-check this with current implementation in Wolfe; its also easy for ``A implies not B''; for more complicated formulae you would resort to backprop through structure of the formula (should I mention this here already?); should mention that this also works for unary relations and entities (but not formulae with mixed unary and binary relations)}
}



% \subsubsection{Product t-Norm}
% \rockt{not sure what to cite for product t-norm}

% In the following a formula $\mathcal{A}$ can not only evaluate to true or false but a probability/confidence, \ie{}, $[\mathcal{A}] \in [0,1]$. 
% It holds that $[\text{true}] := 1$ and $[\text{false}] := 0$. 

% It is conceptually easy to generalize this approach to more complex
% logical formulae involving negation, conjunctions, existential
% quantifiers etc. We only need to derive the gradients of such
% statements. 
% \todoc{This is of course not to say embeddings are guaranteed to capture the intended behavior.} 
% Instead of calculating
% the gradient of this large conjunction, we opt for the easier choice
% of adding all propositional statements to $K$, yielding one term per
% $p$ in equation \ref{obj}.   

% Now we only need the gradient for the propositional statement $\mathcal{F} =
% R_1(p) \lImp R_2(p)$.  This again is straightforward to calculate. For
% example,
% \[\partial/\partial \emb{R_1} = \left(\left(\denote{\lImp} \times_2 \denote{R_2(p)}\right)\boldsymbol{\hat{\eta}}_\lForm\right)\otimes\emb{p}.\]

% we define an objective over the sum of propositional constraints
% with 
% \[\denote{\mathcal{F}_p} \defeq \denote{R_1(p) \lImp R_2(p)} = \top.\]
% % One might be tempted to use $\mathcal{F} = \bigwedge_p \mathcal{F}_p$ instead, but this would amount to a chained tensor-vector product and complicate the gradient derivation. \todoc{I would loose the previous sentence...it is not that necessary}
% It is straight-forward to derive gradients for each summand in the propositionalized version of a first-order constraint. For example,
% \[\partial/\partial \emb{R_1} = \left(\left(\denote{\lImp} \times_2 \denote{R_2(p)}\right)\boldsymbol{\hat{\eta}}\right)\otimes\emb{p}.\] %footnote{Gradients for $\denote{R_2}$ and $\denote{p}$ can be found at \todo.}
% % \todoc{av: hard to follow}
% \todoc{\ie{}, to update the embedding of the relation on the right-hand side of the implication, the overall score of the implication, the score of the left-hand side and the embedding of the argument are used.\todoc{if more space is needed, this can be discarded -- this is just repeating what the equation states}}
% \todoc{Why are we only talking about implication. we should at least
% mention others. also, $\exists$?}


\todo{backprop through logical formulae is very related to backprop through structure by \citep{goller1996learning}}





\subsection{Analysis of Asymmetry in the Predictions}
\label{sec:results:assymm}

\comment{
\subsubsect{Reasoning over Unknown Facts}
%\rockt{what makes joint optimization superior? we get pre-inference when only adding terms over observed premises; It looks like the actual power of low-rank logic comes from adding terms to the objective that enforce consistency over unobserved cells.}

When switching of sampling of entity-pairs for which the premise and the consequent is unobserved in the joint optimization model we get $0.32$ wMAP, which resembles pre-factorization inference performance.
Hence, a key property that makes joint optimization favorable over the other methods is its capability to enforce logic consistency over unobserved atoms, 
which goes beyond generating additional training data. 
\todoc{why? maybe if you generate them in the right way with the right weight for pre-inference, you get the same behavior!?}
For instance, assume the two atoms $r_s(e_i,e_j)$ and $r_t(e_i,e_j)$ are not in the training data and during optimization in one epoch the model's  prediction is $1.0$ for the former and $0.5$ for the latter.
Having a formula $r_s(e_i,e_j) \Rightarrow r_t(e_i,e_j)$ as term in the objective will push the prediction of $r_t(e_i,e_j)$ to $1.0$ as well.
}

%\subsubsect{Asymmetric Reasoning}
\comment{
\begin{table}[t!]
  \centering
%\resizebox{0.9\columnwidth}{!}{
{\small
  \begin{tabular}{llllll}
    \toprule
    & & MF & Pre & Joint\\
    \midrule
    Injected & $r_s \Rightarrow r_t$ & $0.94$ & $0.96$ & $0.97$ \\
    Inverse & $r_t \Rightarrow r_s$ & $0.81$ & $0.83$ & $0.49$\\ 
    %Angle between $\emb{r_s}$ and $\emb{r_t}$ & $25.5\degree$ & $19.5\degree$ & $43.3\degree$\\
    %$\|\emb{r_t}\|_2 - \|\emb{r_s}\|_2$  & $0.09$ & $0.12$ & $-0.11$\\
    \bottomrule
  \end{tabular}
}
%}
  \caption{\small\textbf{Asymmetry in Predictions:} Degree of agreement of the rule, and it's inverse, on the predicted facts.}
  \label{tab:results-asymmetry}
 % \vskip -4mm
\end{table}
}

Since the injected formulae are of the form $\forall x,y: r_s(x,y)\simpl r_t(x,y)$, it is worthwhile to study the extent to which these rules are captured, and which approaches are in fact capturing the asymmetric nature of the implication. % of this information.
To this end, we compute the probabilities that the formulae and their inverse hold, averaged over all annotated formulae and cells.
The degree to which $r_s \simpl r_t$ is captured is quite high for all models ($0.94$, $0.96$, and $0.97$ for matrix factorization, pre-factorization inference, and joint optimization respectively).
On the other hand, the probability of $r_t \simpl r_s$ is also relatively high for matrix factorization and pre-factorization inference ($0.81$ and $0.83$ respectively), suggesting that these methods are primarily capturing symmetric similarity between relations.
Joint optimization, however, produces much more asymmetric predictions (probability of $r_t \simpl r_s$ is $0.49$), demonstrating that it is appropriate for encoding logic in the embeddings. % 
%The degree of asymmetry for matrix factorization ( for  vs. $0.81$ for $r_t \simpl r_s$) and pre-factorization inference ($0.96$ vs. $0.83$) is low, suggesting that these methods are primarily capturing symmetric similarity between relations.
%Joint optimization, however, produces much more asymmetric predictions ($0.97$ vs. $0.49$), demonstrating that it is appropriate for encoding logic in the embeddings. % formulae.

%As we can see in Table~\ref{tab:results-asymmetry}, all the methods seem to capture the forward conditional quite accurately, however when we look at the the \emph{inverse} implication holds, we see that both Pre and MF are enforcing it, suggesting that they are not 


%Furthermore, we measure the difference in length between consequent and premise, and the angle between them.

%Matrix factorization captures asymmetry, but only weakly.
%Pre-factorization inference makes the relation embeddings and predictions actually more symmetric.
%Joint Optimization makes the predictions asymmetric but does this against our intuition. 
%\rockt{explanation in the next section...}


\comment{
\subsubsect{Memorization in Entity-Pair Embeddings}
%\todoc{this would benefit from additional experiments, e.g., analytical updates on relation embeddings}

Joint optimization makes the embeddings of the premise and the consequent more dissimilar, which goes against our intuition how embeddings can capture asymmetric reasoning presented in \S~\ref{sec:bg:logicmf}.
From this we conclude that the only way the formulae are captured in this model is via memorization in the entity-pair embeddings.
This is a phenomena that does not reflect the first-order nature of the formulae, but seems to work well in practice.
\rockt{we performed some follow-up experiments...}
}


==> 5_legacy.tex <==

\section{Differentiable Backward Chaining}
\begin{figure}[h!]
  \centering
    \includegraphics[width=0.8\textwidth]{figures/4/overview}
    \caption{Overview of differentiable backward chaining.}% with \ntpor{} (a) and \ntpand{} (b and c) networks.}
    \label{fig:ntp}    
\end{figure}

\label{sec:dbc}
Backward chaining as in \autoref{alg:backchain} works with one-hot representations of symbols.
That is, the symbols \rel{grandfatherOf} and \rel{grandpaOf} or \eone{} and \efive{} do not share any information.
However, machine learning algorithms can take advantage of the many correlations between relation and entity symbols in large \glspl{KB}.
For example, we might observe that ground atoms with the predicates \rel{grandfatherOf} and \rel{grandpaOf} are often true for the same entity pairs.
Likewise, for many entity pairs we might find that whenever \rel{grandfatherOf} is true, \rel{grandparentOf} is likely also true.

We are interested in constructing a neural network that functions like the backward chaining algorithm in \autoref{alg:backchain}.
It operates on vector representations of symbols and is end-to-end differentiable, which means that we can learn symbol representations directly from \glspl{KB} facts via gradient descent.
This allows us to capture similarities in a vector space.
Furthermore, it will allow us to induce a latent logic program, \ie{}, to learn latent rules of predefined structure.
 

\subsection{Goal and Substitution Structures}
The key idea behind the proof-of-concept NTP presented here is to recursively construct a neural network by replacing operations on symbols in backward chaining with differentiable operations on distributed representations. 
To build such a network we separate goals and substitutions into \emph{vector representations} of involved predicates and constants, and \emph{structures} that define the connections of a neural network. 

For instance, $G=\varg{1}(\varg{2}, \var{X})$ is an example of a structure of an entire \emph{class} of goals. This structure encodes that such goals encompass a vector representation of a predicate symbol $\varg{1}$ and the first argument of the predicate $\varg{2}$. For example, the goal $\rel{grandpaOf}(\efive, \var{X})$ can be specified by $G$ and vector representations $\vect{g}=[\vect{v}_{\rel{grandpaOf}}, \vect{v}_\efive]$. Furthermore, based on the structure $G$ it is clear that proofs of that goal will be substitutions for $\var{X}$ (\eg{} $\vect{v}_\ethree$).
%For instance, $G=\varg{1}(\varg{2}, \var{X})$ defines the structure of an entire \emph{class} of queries that given two vectors (one representing a predicate and the other a constant for the first argument, \eg{}, $\vect{g}=[\vect{v}_\rel{grandpaOf}, \vect{v}_\efive]$) returns  representations of other constants that can be substituted for \var{X} (\eg{} $\vect{v}_\ethree$). 
%We divide such substitutions into a structure (\eg{} $S = \{\var{X}/\varg{1}\}$), representations that are compliant with this structure (\eg{}, $\mathbf{s} = [\vect{v}_\ethree]$), as well as a real-valued score $\success \in (0,1)$ that measures the success of the substitution.
Akin to goals, we divide substitutions into structures and representations, as well as a scalar score $\subsuccess \in (0,1)$ that measures the success of the substitution.
For example, proofs of goals of the structure $G$ as defined above will be substitutions with the structure $S = \{\var{X}/\varg{1}\}$ accompanied by substitution representations %compatible with this structure
(\eg{} $\mathbf{s} = [\vect{v}_\ethree]$).

With this divide we can now redefine operations in backward chaining as follows. 
Operations that concern variables and rules are mapping goal and substitution structures ($G$ and $S$) to new structures that instantiate sub-networks.
In contrast, operations on symbols of predicates and constants can be computed in vector space in a differentiable manner, and thus correspond to activations in the neural network. 
The resulting recursively constructed NTP is end-to-end differentiable.
An overview of the model architecture with an example is given in Figure~\ref{fig:ntp} and discussed in detail below.

%Hard-wired connections in this network are instantiated based on the structure of rules in a KB, the structure of a class of queries, as well as operations on these structures.
%As such, the NTP introduced here closely follows the steps of symbolic backward chaining, but less restricted architectures that replace operations in the NTP with parameterized functions are possible as well. 

\subsection{\ntpor{}}
The entry point to the NTP is an \ntpor{} network (Figure \ref{fig:ntp}a) that for a given goal and substitution structure ($G$ and $S$) instantiates a sub-network for each one of the $N$ rules in a knowledge base $T$.
The unification of the $i$th rule's right-hand side with a goal structure results in a new substitution structure $S_i$. 
When provided with a goal representation, a unification network is computing the unification success in vector space.
For example, assume at some proof-depth $D$ in the \gls{NTP} we unify $\rel{grandfatherOf}(\eone, Q)$ with $\rel{grandpaOf}(\efive, \etwo)$. This will result in a new substitution structure $S'_i=\{Q/\varg{1}\}$, representation $\vect{s} = [\vect{v}_{\etwo}]$ and success $\subsuccess^D$ that is passed further in the network. In contrast to discrete unification that checks for symbol equality, we calculate a soft unification from the previous unification success of the outer network $\subsuccess^{D+1}$ and the similarity of predicate and constant representations. For instance, for the unification example above we obtain:
\begin{align}
\subsuccess_{\text{predicate}} &= \text{sigmoid}(\vect{v}^T_{\rel{grandfatherOf}}\vect{v}_{\rel{grandpa}})\\
\subsuccess_{\text{arg}_1} &= \text{sigmoid}(\vect{v}^T_{\eone}\vect{v}_{\efive})\\
\subsuccess^D &= \min(\subsuccess^{D+1}, \subsuccess_{\text{predicate}}, \subsuccess_{\text{arg}_1})\label{eq:succ}
\end{align}
%Note that soft-unification of symbol representations could also be parameterized and learned by a deep feed-forward neural network.




\subsection{\ntpand{}}
The new substitution structure calculated by unification instantiates an \ntpand{} network (Figure \ref{fig:ntp}c) at depth $D$ that attempts to sequentially prove the left-hand side atoms of the rule given the current substitutions. 
If the rule's left-hand side structure is empty (\eg{} when the right-hand side represents a fact in the \gls{KB}) the \ntpand{} network simply passes the substitutions and their success through (Figure \ref{fig:ntp}b). Otherwise, it applies the substitution on the first atom of the left-hand side, resulting in a new goal structure and representation, and instantiates an \ntpor{} network with that structure and the previous substitution.

For example, assume unify the head of $\rel{fatherOf}(X,Y)$ $\wedge$ $\rel{parentOf}(Y,Z)$ $\Rightarrow$ $\rel{grandfatherOf}(X,Z)$ with the goal $\rel{grandfatherOf}(\eone, Q)$. 
The result is a unification success $\subsuccess^D$ as calculated in Eq. \ref{eq:succ}, as well as a new substitution structure $S = \{Q/Z, X/\varg{1}\}$ where $\vect{s} = [\vect{v}_{\eone}]$ becomes the input to the \ntpand{} network. 
This network will first apply the substitution to $\rel{fatherOf}(X,Y)$, resulting in a new goal structure $G' = \varg{1}(\varg{2},Y)$. 
This structure now instantiates another \gls{NTP} (\ie{} an \ntpor{} module) of depth $D-1$, which attempts to prove the input goal representation $\vect{g} = [\vect{v}_{\rel{fatherOf}}, \vect{v}_{\eone}]$.

For every proof, \ie{}, every possible substitution of the structure $S' = \{Q/Z, Y/\varg{1}\}$, a new \ntpand{} module is instantiated that attempts to recursively prove the remainder of the left-hand side ($\rel{parentOf}(Y,Z)$ in the example above). Finally, the successes of all identical substitutions (\ie{} substitutions to the same variables or representations of constants) are merged by taking their max.

Note that given a KB, goal structure and depth, the network structure of the NTP is fully specified and many goals of the same structure can be used to perform training and inference with the NTP. 

%Furthermore, note that in the example above the network processes vector representations of symbols that are known, so we could instead simply process symbols that are only transformed into a dense representation when unifying. However, in future work we want to experiment with NTPs that alter symbol representations during processing or whose input are representations of natural language statements instead of symbols.

\subsection{Trainable Rules}
NTPs are not only differentiable with respect to symbol representations in the KB, but also latent symbol representations in first-order rules of predefined structure. For instance, we could assume that for some predicates in a KB a transitive relationship holds. We can define a rule template $\varg{1}(X,Y) \wedge \varg{1}(Y,Z) \Rightarrow \varg{2}(X,Z)$ whose latent predicates $\vect{v}_{\varg{1}}, \vect{v}_{\varg{2}}$ are trainable parameters and optimized in the same way as symbol representations.


%\subsection{Provenance by Proof}
%\label{sec:proofs}
%\tim{move this into introduction}
%As opposed to less structured neural architectures, NTPs allow for provenance by inspection of proofs. Concretely, we can trace the transformations that led to an output substitution with maximal score through the neural network and inspect the resulting proof. Such a proof may contain applications of latent formulae, which can be inspected by retrieving for every latent predicate the most similar known predicate representation.

\section{Results and Discussion}
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/4/results}
    \caption{Predictions of different NTP modes on a toy KB where every column (within a subplot) represents a predicate and every row an entity-pair. Training facts (red) and test facts (blue) in the first subplot are consistent with two rules: $r_1(X,Y) \wedge r_1(Y,Z) \Rightarrow r_2(X,Z)$ and 
    $r_3(X,Y) \wedge r_4(X,Y) \Rightarrow r_5(X,Y)$. The other three subplots show predictions between 0 (white) and 1 (black) of the different modes discussed in text.} %\Seb{Describe columns in figure here as well.}
    \label{fig:res}
\end{figure}

We implemented an NTP with differentiable backward chaining in TensorFlow~\citep{abadi2015tensorflow}. Symbol representations are initialized randomly and constrained to unit-length.
During training we iterate over the set of known facts, and optimize negative log-likelihood of the proof success of every fact based on all other facts (and rules) using Adam \citep{kingma2015adam}. 
Furthermore, for every training fact we sample an unobserved fact for the same predicate (but different entity-pair) and optimize its proof with a target success of zero.

Our NTP implementation is tested on toy KBs for different scenarios shown in the four different subplots in Figure \ref{fig:res}. Every column (within a subplot) represents a predicate and every row an entity-pair.
First, we run the NTP with given ground-truth rules without training symbol or rule representations, and test whether it can act as a discrete theorem prover. As expected, given rules the NTP can infer all test facts (2nd subplot in Figure \ref{fig:res}).
The third subplot shows predictions when we let the NTP try to reconstruct training facts only with the help of other facts by learning symbol representations (similar to other representation learning approaches for KB inference).
Finally, a core benefit of the NTP is visible once we provide few reasonable rule templates\footnote{We use $\varg{1}(X,Y) \Rightarrow \varg{2}(X,Y)$, $\varg{1}(X,Y) \wedge \varg{2}(X,Y) \Rightarrow \varg{3}(X,Y)$ and $\varg{1}(X,Y) \wedge \varg{1}(Y,Z) \Rightarrow \varg{2}(X,Z)$.} and optimize for rule representations that best explain observed facts (4th subplot). 
%\Seb{Could omit the next two sentences} 
We found that this can work remarkably well, but also noticed that the quality of trained rules is varying with different random initialization of the rule's parameters. We need to investigate in future work how the robustness of rule learning in NTPs can be improved.





%%% Local Variables:
%%% TeX-master: "thesis"
%%% End:

